Analysis and Evaluation of Language Models for Word Sense Disambiguation

Transformer-based language models have taken many fields in NLP by storm. BERT and its derivatives dominate most of the existing evaluation benchmarks, including those for Word Sense Disambiguation (WSD), thanks to their ability in capturing context-sensitive semantic nuances. However, there is still little knowledge about their capabilities and potential limitations in encoding and recovering word senses. In this article, we provide an in-depth quantitative and qualitative analysis of the celebrated BERT model with respect to lexical ambiguity. One of the main conclusions of our analysis is that BERT can accurately capture high-level sense distinctions, even when a limited number of examples is available for each word sense. Our analysis also reveals that in some cases language models come close to solving coarse-grained noun disambiguation under ideal conditions in terms of availability of training data and computing resources. However, this scenario rarely occurs in real-world settings and, hence, many practical challenges remain even in the coarse-grained setting. We also perform an in-depth comparison of the two main language model based WSD strategies, i.e., fine-tuning and feature extraction, finding that the latter approach is more robust with respect to sense bias and it can better exploit limited available training data. In fact, the simple feature extraction strategy of averaging contextualized embeddings proves robust even using only three training sentences per word sense, with minimal improvements obtained by increasing the size of this training data.

==> OLD_TABLES.tex <==

\begin{figure*}[t!]
\begin{center}
		%\includegraphics[trim = 0mm 0mm 0mm 0mm,,scale=0.37]{Figure_EMNLP_paper.png}
		%\includegraphics[trim = 0mm 0mm 0mm 0mm,,scale=0.238]{Figure_EMNLP_paper.png}
		%[scale=0.325]
		%width=\textwidth,
		\includegraphics[scale=0.64,angle=0]{images/detailed.png}
%scale=0.235
\end{center}
    \caption{Heatmap indicating the recall of BERT (fine-tuning) on all senses for each word. Percentages indicate different training data sizes. \green{To remove?}  %\red{Font size very small for the 100\% experiment}
    }
    \label{fig:balancedfull}
\end{figure*}

\begin{figure}[ht]
    \centering
    \includegraphics[width=7.8cm]{nshot2.png}
    \caption{$N$-shot learning results for fine-tuned BERT-Base. $N$ is the number of training instances per sense. \red{X-axis is at a logarithmic scale?} \green{Will we keep this?}}
    \label{fig:galaxy}
\end{figure}


\begin{table}[h]
\setlength{\tabcolsep}{12.0pt}
%\scalebox{0.9}{
%\resizebox{\columnwidth}{!}{%
%\small
\begin{tabular}{lcccc@{\hskip 20pt}cccc}
\toprule
 &
\multicolumn{4}{c@{\hskip 20pt}}{\bf Macro F1} &
\multicolumn{4}{c}{\bf Micro F1} \\
\cmidrule(lr@{\hskip 20pt}){2-5}
\cmidrule(lr){6-9}
&
\multicolumn{1}{c}{\bf 1}   &
\multicolumn{1}{c}{\bf  3}  &
\multicolumn{1}{c}{\bf 10} &
\multicolumn{1}{c@{\hskip 20pt}}{\bf 30} &
\multicolumn{1}{c}{\bf 1}   &
\multicolumn{1}{c}{\bf  3}  &
\multicolumn{1}{c}{\bf 10} &
\multicolumn{1}{c}{\bf 30} \\  

 
\midrule

chair	& 40.4 &	94.5 &	95.5 &	96.4 & 54.6 &	95.3 &	96.1 &	96.9 \\
apple   & 57.0 & 98.9 & 	97.0 &	99.2 & 55.1 &	98.9 &	97.1 &	99.2 \\
java	& 98.8	 & 99.5 & 	97.9 &	98.9 & 98.9 &	99.5 &	98.0 &	99.0 \\
crane	& 64.6	& 93.6	& 86.5 & 	93.6 & 65.0 &	93.6 &	86.4 &	93.6 \\
bass	& 21.5 &	56.8 &	67.0 &	78.3 & 16.8 &	68.7 &	80.2 &	89.8\\
bow		& 73.4 &	87.3 &	88.3 &	92.8 & 78.0	& 89.1 &	89.5 &	93.9 \\
square	& 59.3 &	80.8 &	85.0 &	90.6 & 59.5 &	88.0 &	90.3 &	94.6 \\
seal	& 71.1 &	85.4 &	91.8 &	92.1 & 70.1 &	93.4 &	94.5 & 96.3 \\

\midrule
average     & 60.8 &	87.1 &	88.6 &	92.7 & 62.3 &	90.8 &	91.5 &	95.4s \\
\bottomrule
\end{tabular}
%}
\caption{$N$-shot learning results for fine-tuned BERT-Base. The numbers on top indicate the number of training instance per sense.} %Notation is similar to Table \ref{tab:evCoarseWSD}.} %FT stands for Fine-tune.}
\label{tab:nshot-table}
\end{table}

\begin{table}[t]
\setlength{\tabcolsep}{5.4pt}
\renewcommand{\arraystretch}{1.02}
%\scalebox{0.77}{
\small
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllllll@{\hskip 10pt}llllll}
\toprule
\multirow{2}{*}{\textbf{Word}} &
\multicolumn{6}{c@{\hskip 10pt}}
{\bf Most frequent class} &
\multicolumn{6}{c}{\bf Least frequent class} \\ 
\cmidrule(lr@{\hskip 10pt}){2-7}
\cmidrule(lr){8-13}
& \multicolumn{1}{c}{All} & 50\% & 25\% & 10\% & 5\% & 1\% & \multicolumn{1}{c}{All} & 50\% & 25\% & 10\% & 5\% & 1\% \\
 \midrule
crane & \cellcolor{c1!75} 98.8 & \cellcolor{c1!100} 100 & \cellcolor{c1!75} 98.8 & \cellcolor{c1!75} 98.8 & \cellcolor{c2!10} 90.1 & \cellcolor{c1!100} 100 & \cellcolor{c1!21} 96.1 & \cellcolor{c2!12} 89.5 & \cellcolor{c2!9} 90.8 & \cellcolor{c2!9} 90.8 & \cellcolor{c1!100} 100 & \cellcolor{c2!41} 76.3  \\
java & \cellcolor{c1!95} 99.8 & \cellcolor{c1!88} 99.4 & \cellcolor{c1!94} 99.7 & \cellcolor{c1!98} 99.9 & \cellcolor{c1!98} 99.9 & \cellcolor{c1!88} 99.4 & \cellcolor{c1!54} 97.7 & \cellcolor{c1!94} 99.7 & \cellcolor{c1!84} 99.2 & \cellcolor{c1!70} 98.5 & \cellcolor{c1!61} 98.1 & \cellcolor{c1!94} 99.7  \\
apple & \cellcolor{c1!95} 99.8 & \cellcolor{c1!94} 99.7 & \cellcolor{c1!94} 99.7 & \cellcolor{c1!94} 99.7 & \cellcolor{c1!78} 98.9 & \cellcolor{c1!90} 99.5 & \cellcolor{c1!54} 97.7 & \cellcolor{c1!74} 98.7 & \cellcolor{c1!70} 98.5 & \cellcolor{c1!70} 98.5 & \cellcolor{c1!70} 98.5 & \cellcolor{c1!54} 97.7  \\
mole & \cellcolor{c1!100} 100 & \cellcolor{c1!74} 98.7 & \cellcolor{c1!100} 100 & \cellcolor{c1!74} 98.7 & \cellcolor{c1!21} 96.1 & \cellcolor{c2!52} 71.4 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c2!55} 70.0 & \cellcolor{c2!22} 85.0 & \cellcolor{c2!66} 65.0  \\
spring & \cellcolor{c1!50} 97.5 & \cellcolor{c1!65} 98.3 & \cellcolor{c1!5} 95.3 & \cellcolor{c2!2} 94.1 & \cellcolor{c1!5} 95.3 & \cellcolor{c2!20} 86.0 & \cellcolor{c1!45} 97.3 & \cellcolor{c1!45} 97.3 & \cellcolor{c1!45} 97.3 & \cellcolor{c1!71} 98.6 & \cellcolor{c1!45} 97.3 & \cellcolor{c2!4} 93.2  \\
chair & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!78} 98.9 & \cellcolor{c1!78} 98.9 & \cellcolor{c1!100} 100 & \cellcolor{c2!26} 83.0 & \cellcolor{c2!10} 90.5 & \cellcolor{c2!10} 90.5 & \cellcolor{c2!10} 90.5 & \cellcolor{c2!10} 90.5 & \cellcolor{c2!26} 83.3 & \cellcolor{c1!51} 97.6  \\
hood & \cellcolor{c1!58} 97.9 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c2!6} 92.3 & \cellcolor{c2!23} 84.6 & \cellcolor{c2!40} 76.9 & \cellcolor{c2!6} 92.3 & \cellcolor{c2!100} 0.0  \\
seal & \cellcolor{c1!70} 98.5 & \cellcolor{c1!54} 97.7 & \cellcolor{c1!24} 96.2 & \cellcolor{c1!84} 99.2 & \cellcolor{c1!70} 98.5 & \cellcolor{c1!70} 98.5 & \cellcolor{c2!7} 91.7 & \cellcolor{c1!100} 100 & \cellcolor{c2!7} 91.7 & \cellcolor{c2!7} 91.7 & \cellcolor{c2!7} 91.7 & \cellcolor{c2!100} 33.3  \\
bow & \cellcolor{c1!81} 99.1 & \cellcolor{c1!48} 97.4 & \cellcolor{c1!81} 99.1 & \cellcolor{c1!65} 98.3 & \cellcolor{c1!31} 96.6 & \cellcolor{c1!14} 95.7 & \cellcolor{c1!24} 96.2 & \cellcolor{c1!100} 100 & \cellcolor{c2!23} 84.6 & \cellcolor{c2!23} 84.6 & \cellcolor{c2!6} 92.3 & \cellcolor{c2!100} 11.5  \\
club & \cellcolor{c2!34} 79.6 & \cellcolor{c2!32} 80.6 & \cellcolor{c2!30} 81.5 & \cellcolor{c2!26} 83.3 & \cellcolor{c2!40} 76.9 & \cellcolor{c2!11} 89.8 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c2!10} 90.5 & \cellcolor{c2!94} 52.4 & \cellcolor{c2!10} 90.5 & \cellcolor{c2!100} 47.6  \\
trunk & \cellcolor{c1!14} 95.7 & \cellcolor{c1!100} 100 & \cellcolor{c1!58} 97.9 & \cellcolor{c1!100} 100 & \cellcolor{c1!14} 95.7 & \cellcolor{c1!58} 97.9 & \cellcolor{c1!100} 100 & \cellcolor{c2!36} 78.6 & \cellcolor{c2!20} 85.7 & \cellcolor{c1!100} 100 & \cellcolor{c2!84} 57.1 & \cellcolor{c2!100} 50.0  \\
square & \cellcolor{c1!41} 97.1 & \cellcolor{c1!80} 99.0 & \cellcolor{c1!21} 96.1 & \cellcolor{c2!6} 92.2 & \cellcolor{c1!61} 98.1 & \cellcolor{c2!27} 82.5 & \cellcolor{c2!23} 84.6 & \cellcolor{c2!100} 23.1 & \cellcolor{c2!100} 7.7 & \cellcolor{c2!100} 15.4 & \cellcolor{c2!100} 30.8 & \cellcolor{c2!100} 38.5  \\
arm & \cellcolor{c1!84} 99.2 & \cellcolor{c1!84} 99.2 & \cellcolor{c1!84} 99.2 & \cellcolor{c1!50} 97.5 & \cellcolor{c1!84} 99.2 & \cellcolor{c1!84} 99.2 & \cellcolor{c1!100} 100 & \cellcolor{c1!54} 97.7 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!54} 97.7 & \cellcolor{c1!100} 100  \\
digit & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c2!38} 77.8 & \cellcolor{c2!38} 77.8 & \cellcolor{c2!62} 66.7 & \cellcolor{c2!62} 66.7  \\
bass & \cellcolor{c1!65} 98.3 & \cellcolor{c1!75} 98.8 & \cellcolor{c1!54} 97.7 & \cellcolor{c1!68} 98.4 & \cellcolor{c1!78} 98.9 & \cellcolor{c1!71} 98.6 & \cellcolor{c2!84} 56.8 & \cellcolor{c2!79} 59.1 & \cellcolor{c2!82} 58.0 & \cellcolor{c2!100} 40.9 & \cellcolor{c2!100} 31.8 & \cellcolor{c2!100} 15.9  \\
yard & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c2!17} 86.9 & \cellcolor{c1!1} 95.1 & \cellcolor{c2!3} 93.4 & \cellcolor{c1!100} 100 & \cellcolor{c2!9} 90.9 & \cellcolor{c2!100} 45.5 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c2!49} 72.7  \\
pound & \cellcolor{c1!54} 97.7 & \cellcolor{c1!78} 98.9 & \cellcolor{c1!78} 98.9 & \cellcolor{c1!78} 98.9 & \cellcolor{c1!100} 100 & \cellcolor{c2!22} 85.1 & \cellcolor{c1!100} 100 & \cellcolor{c2!77} 60.0 & \cellcolor{c2!100} 20.0 & \cellcolor{c2!100} 10.0 & \cellcolor{c2!100} 10.0 & \cellcolor{c2!100} 20.0  \\
deck & \cellcolor{c1!78} 98.9 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!55} 97.8 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c2!52} 71.4 & \cellcolor{c2!84} 57.1 & \cellcolor{c2!84} 57.1 & \cellcolor{c2!84} 57.1 & \cellcolor{c2!100} 0.0 & \cellcolor{c2!100} 0.0  \\
bank & \cellcolor{c1!95} 99.8 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!75} 98.8 & \cellcolor{c1!100} 100 & \cellcolor{c2!19} 86.4 & \cellcolor{c2!29} 81.8 & \cellcolor{c2!19} 86.4 & \cellcolor{c2!39} 77.3 & \cellcolor{c1!10} 95.5 & \cellcolor{c2!100} 9.1  \\
pitcher & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c1!100} 100 & \cellcolor{c2!57} 69.2 & \cellcolor{c2!100} 20.0 & \cellcolor{c2!91} 53.8 & \cellcolor{c2!74} 61.5 & \cellcolor{c2!100} 15.4 & \cellcolor{c2!91} 53.8	\\
\end{tabular}%
%}
%}
\caption{Recall performance for fine-tuned BERT with different training data sizes on the most and least frequent classes for each word. Words sorted by entropy.}
\label{tab:most-least}
\end{table}



\begin{table}[t]
\setlength{\tabcolsep}{16.0pt}
\renewcommand{\arraystretch}{0.95}
%\scalebox{0.78}{
%\resizebox{\columnwidth}{!}{%
%\small
\begin{tabular}{l rr|rr|rr}
\toprule

&
\multicolumn{2}{c}{\bf Micro F1}   &
\multicolumn{2}{c}{\bf  Macro-P}  &
\multicolumn{2}{c}{\bf  Macro-R}\\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
&   \multicolumn{1}{c}{SKW}	&   \multicolumn{1}{c}{BAL} &
\multicolumn{1}{c}{SKW}	&   \multicolumn{1}{c}{BAL} &
\multicolumn{1}{c}{SKW}	&   \multicolumn{1}{c}{BAL} \\
\midrule
crane	&	\textbf{97.5}	&	\textbf{97.5}	&	\textbf{97.4}	&	\textbf{97.4}	&	\textbf{97.5}	&	\textbf{97.5} \\
java	&	99.0	&	\textbf{99.3}	&	98.8	&	\textbf{99.3}	&	\textbf{99.2}	&	\textbf{99.2} \\
apple	&	\textbf{99.0}	&	98.1	&	\textbf{98.8}	&	98.2	&	\textbf{99.2}	&	97.8 \\
mole	&	\textbf{99.5}	&	98.5	&	\textbf{99.5}	&	98.4	&	\textbf{99.7}	&	99.0 \\
spring	&	\textbf{97.8}	&	97.6	&	\textbf{97.8}	&	97.6	&	\textbf{97.1}	&	\textbf{97.1} \\
chair	&	\textbf{96.9}	&	95.4	&	\textbf{95.2}	&	94.1	&	\textbf{97.8}	&	95.3 \\
hood	&	94.0	&	\textbf{97.5}	&	93.2	&	\textbf{95.9}	&	91.4	&	\textbf{97.8} \\
seal	&	\textbf{98.6}	&	97.6	&	97.1	&	\textbf{98.1}	&	\textbf{98.9}	&	91.8 \\
bow	    &	97.7	&	\textbf{98.6}	&	97.0	&	\textbf{99.0}	&	\textbf{97.2}	&	\textbf{97.2} \\
club	&	\textbf{82.6}	&	82.2	&	\textbf{87.3}	&	86.4	&	\textbf{80.6}	&	78.8 \\
trunk	&	\textbf{97.5}	&	96.1	&	\textbf{98.6}	&	96.5	&	\textbf{95.8}	&	95.0 \\
square	&	\textbf{95.6}	&	91.9	&	92.0	&	\textbf{95.0}    &	\textbf{96.3}	&	84.5 \\
arm	    &	\textbf{99.4}	&	\textbf{99.4}	&	\textbf{99.6}	&	\textbf{99.6}	&	\textbf{98.9}	&	\textbf{98.9} \\
digit	&	\textbf{100}	    &	\textbf{100} 	&	\textbf{100}	    &	\textbf{100}	    &	\textbf{100}	    &	\textbf{100} \\
bass	&	\textbf{94.8}	&	93.4	&	83.6	&	\textbf{89.8}	&	\textbf{90.7}	&	81.8 \\
yard	&	\textbf{100}	    &	92.3	&	\textbf{100}	    &	95.1	&	\textbf{100}	    &	82.4 \\
pound	&	\textbf{98.0}	&	82.4	&	\textbf{98.9}	&	87.9	&	\textbf{91.7}	&	66.1 \\
deck	&	96.9	&	\textbf{99.0}    &	85.2	&	\textbf{99.5}	&	90.6	&	\textbf{93.8} \\ 
bank	&	\textbf{99.1}	&	92.3	&	93.1	&	\textbf{94.8}	&	\textbf{97.2}	&	66.4 \\
pitcher	&	\textbf{99.8}	&	99.1	&	84.6	&	\textbf{99.3}	&	\textbf{99.9}	&	63.0 \\
\midrule
AVG	    &	\textbf{97.2}	&	95.4	&	94.9	&	\textbf{96.1}	&	\textbf{96.0}	&	89.2 \\
\end{tabular}
%}
\caption{WSD performance of BERT\red{-L??} fine-tuned for the original skewed (SKW) and balanced (BAL) training sets (evaluated on the same original skewed test set), in terms of macro precision (Macro-P), and recall (Marco-R), as well as micro F1. Words sorted by entropy. \red{Add also 1NN results?}}
\label{tab:balanced}
\end{table}
